Session Guarantees with Raft and Hybrid Logical Clocks

Eventual consistency is a popular consistency model for geo-replicated data stores. Although eventual consistency provides high performance and availability, it can cause anomalies that make programming complex for application developers. Session guarantees can remove some of these anomalies while causing much lower overhead compared with stronger consistency models. In this paper, we provide a protocol for providing session guarantees for NuKV, a key-value store developed for services with very high availability and performance requirements at eBay. NuKV relies on the Raft protocol for replication inside datacenters, and uses eventual consistency for replication among datacenters. We provide modified versions of conventional session guarantees to avoid the problem of slowdown cascades in systems with large numbers of partitions. We also use Hybrid Logical Clocks to eliminate the need for delaying write operations to satisfy session guarantees. Our experiments show that our protocol provides session guarantees with a negligible overhead when compared with eventual consistency.

==> Notes.tex <==
5/30/2018: 

- For comparison, we can compare with quorum techniques to provide read-your-write, or other methods. 

- Important: I think monotonic write and write-follows-read is only useful for write operations that read the current value and modify it, like increment, or more complex write operations. For simple PUT, monotonic write or write-follows-read has no meaning. 


==> dkv.tex <==
\subsection{Distributed Key-value Stores}
Key-value stores provide a simple abstraction to store and retrieve  data. Each key-value store is a set of $\langle key, value \rangle$ pairs. A key-value store has two basic operations: $PUT(k, v)$ and $GET(k)$. $PUT(k, v)$ writes a new version with value $v$ for data item with key $k$, and $GET(k)$ reads the value of the data item with key $k$. 
%Key-value stores are the basis of document-oriented databases. These databases can handle one-to-many relations more efficiently than relational databases. Specifically, we can encode all pieces of data related to a key as a JSON (or XML) document, and store it as the value for that key in the key-value store. This approach provides better \textit{locality} than multi-table schemas that are normally used in relational databases \cite{book}. 
%
%The schemaless data model of document-oriented databases gives us the freedom from strict schema at the write time, and lets the application interpret the structure of the encoded value at the read time. This also eliminates the need for awkward object-relational mapping layers that we usually need for relational databases. Specifically, we can easily encode/decode fields of an object to/from documents that we store in the database. Many new storage systems such as MongoDB \cite{mongoDB}, RethinkDB \cite{rethinkDB}, CouchDB \cite{couchDB}, and Espresso \cite{espresso} support document-oriented data model. 

Typically, to increase the performance, we must distribute the key-value store. Two main techniques to distribute the data are partitioning and replication. Partitioning (also known as sharding) allows us to store the data in more than one machine. Specifically, we can divide the key space into several parts, and store each part on a different machine. Usually, we partition the data in a way that each key is assigned to exactly one partition. Partitioning increases the scalability of the system, as we do not need to fit the whole key space on a single machine. It also enables us to scale query throughput by adding more nodes \cite{book}. 

Replication, on the other hand, improves durability, availability, and performance. Specifically, by keeping multiple copies of data in several replicas, we can increase the durability of the data. It also improves the availability of the system, as if a replica fails, other replicas can serve the clients. Moreover, using replication, we can keep data geographically close to the clients, thereby reducing the network latency. Because of these benefits, geo-replicated data stores have become an important building block of today's cloud services \cite{cops}.

==> testGraph.tex <==
\begin{figure} [h]
\begin{center}
\begin{tikzpicture}
\begin{axis} [height=6cm, width= \columnwidth, legend pos= north west, grid=both]
\addplot  table[x=threads, y=E_H_L
, col sep=comma] {data/local_prob1.csv};
\addlegendentry{$E_H$}

\addplot  table[x=threads, y=E_L
, col sep=comma] {data/local_prob1.csv};
\addlegendentry{$E$}

\addplot  table[x=threads, y=M_H_L
, col sep=comma] {data/local_prob1.csv};
\addlegendentry{$M_H$}

\addplot table[x=threads, y=M_L
, col sep=comma] {data/local_prob1.csv};
\addlegendentry{$M$}
\end{axis}
\end{tikzpicture}
\caption{The effect of load on latency of mixed PUT and GET operations with locality of traffic.}
\label{fig:local_prob1_latency}
\end{center}
\end{figure}
